Gaussian Process Stochastic Frontiers with Two-Way Fixed Effects

Parametric frontier restrictions and unobserved time heterogeneity can distort efficiency measurement in panel data. This paper develops a Bayesian stochastic frontier model with a Gaussian process prior and unrestricted individual and time effects that may be correlated with inputs. Conditional on inefficiency, orthogonal projection eliminates both sets of fixed effects, yielding a restricted likelihood that retains observation-specific inefficiency. Monte Carlo experiments show competitive performance under correct parametric specification and improved performance when benchmark models impose an incorrect frontier functional form or omit time effects. An application to Spanish dairy farms observed from 1999 to 2010 yields similar average technical efficiency across specifications, but a lower posterior mean of average returns to scale, with greater uncertainty, under the Gaussian process frontier. Models with year effects also yield more stable estimated efficiency profiles than the benchmark with a quadratic trend and time-input interactions. These findings show that conclusions about scale economies and efficiency dynamics depend on both frontier flexibility and the treatment of time heterogeneity.

==> Preamble.tex <==
% Shared preamble copied from the Gaussian Process main (1).tex.
% The document class and xr-hyper are loaded by each driver.
% Duplicate setspace and algorithm loads have been removed.
\usepackage[colon]{natbib}
\usepackage[pdftex,colorlinks=true]{hyperref}
\usepackage{verbatim}  
% Needed for the "comment" environment to make LaTeX comments
\hypersetup{citecolor=blue,linkcolor=blue,urlcolor=blue}
\usepackage{setspace}

%\usepackage[disable=footnote]{microtype}
\usepackage{rotating,multirow,multicol,bm}
\usepackage{lscape,pdflscape}
%\usepackage{unicode-math}
\usepackage{algorithm,algpseudocode}
\usepackage{lipsum}
\usepackage[margin=0.85in]{geometry}
\graphicspath{{Figures/}}
%\usepackage[margin=2cm]{geometry}  % only to bring all on one page
\usepackage{graphicx}
\usepackage{caption, subcaption}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage[title]{appendix}
\usepackage{makecell}
\usepackage{threeparttable}
\usepackage{chngcntr} % 

\usepackage{amsmath,paralist,color,url}
%\usepackage{pifont} 
%\usepackage{utopia}
%\RequirePackage[T1]{fontenc}
\usepackage[charter]{mathdesign}

%\usepackage[demo]{graphicx}
%\usepackage{subcaption}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\Norm}{\mathcal{N}}
\newcommand{\Corr}{\operatorname{Corr}}
\newcommand{\Var}{\operatorname{Var}}

\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{proof}{Proof}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\DeclareCaptionFormat{cont}{#1 (cont.)#2#3\par}


\newcommand\pcite[1]{\citeauthor{#1}'s \citeyearpar{#1}}
\newcommand\ppcite[1]{\citeauthor*{#1}'s \citeyearpar{#1}}
\newcommand\pscite[1]{\citeauthor{#1}' \citeyearpar{#1}}

%\bibliographystyle{elsarticle-harv}
%\bibliographystyle{agsm}
\bibliographystyle{jae}

\title{\vspace{-1.2cm} }
\author{}
\date{ }

% Cross-document references, following the Fourier driver structure.
% Internal links and citations retain the source colors; external PDF links
% are red. Reference snapshots also support a fresh PDFLaTeX build.
\hypersetup{filecolor=red}
\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}%
  \@addtofilelist{#1}%
  \IfFileExists{#1}{}{\typeout{No file #1.}}}
\makeatother
\newcommand*{\myexternaldocument}[2]{%
  \IfFileExists{#1.refs.aux}{%
    \externaldocument[][nocite]{#1.refs}[#2]%
  }{}%
  \IfFileExists{#1.aux}{%
    \externaldocument[][nocite]{#1}[#2]%
  }{}%
  \addFileDependency{#1.tex}%
  \addFileDependency{#1.aux}}

